Convergence Rates for the Generalized Fr\'echet Mean via the Quadruple Inequality

For sets $\mathcal Q$ and $\mathcal Y$, the generalized Fr\'echet mean $m \in \mathcal Q$ of a random variable $Y$, which has values in $\mathcal Y$, is any minimizer of $q\mapsto \mathbb E[\mathfrak c(q,Y)]$, where $\mathfrak c \colon \mathcal Q \times \mathcal Y \to \mathbb R$ is a cost function. There are little restrictions to $\mathcal Q$ and $\mathcal Y$. In particular, $\mathcal Q$ can be a non-Euclidean metric space. We provide convergence rates for the empirical generalized Fr\'echet mean. Conditions for rates in probability and rates in expectation are given. In contrast to previous results on Fr\'echet means, we do not require a finite diameter of the $\mathcal Q$ or $\mathcal Y$. Instead, we assume an inequality, which we call quadruple inequality. It generalizes an otherwise common Lipschitz condition on the cost function. This quadruple inequality is known to hold in Hadamard spaces. We show that it also holds in a suitable way for certain powers of a Hadamard-metric.

==> conclusion.tex <==
\section{Conclusion}
%
For obtaining rates of convergence for the estimator of the generalized Fréchet mean, we introduced the quadruple inequality, which replaces a Lipschitz-con\-ti\-nu\-ity requirement of classical results. We showed that in some spaces, in particular in Hadamard spaces, this allows for better bounds without an otherwise common boundedness requirement.

We showed how three basic ingredients influence the obtained rate: the aforementioned quadruple inequality, a growth condition on the objective function, and an entropy condition.

We proved a power inequality, which is a special type of quadruple inequality that relates powers of distances in metric spaces. We applied it in the Fréchet mean setting, but it might be of interest on its own. 
%
%
